FailPoint-X: A Policy-Matched, Failure-Anchored Benchmark for Offline VLA Post-Training from Human Takeovers

Human takeovers offer corrective supervision for vision-language-action (VLA) policies, but their contribution to offline post-training must be separated from that of continued optimization. We introduce FailPoint-X, a benchmark for offline VLA post-training with human takeovers. To represent uncertainty in failure onset, an annotator marks an interval for each failure, and training takeovers start at seeded frames sampled within it. From one fixed $\pi_{0.5}$ checkpoint, which also initializes post-training, we assemble 629 natural failures across 10 LIBERO-X task families at up to five difficulty levels. All 2,823 takeover attempts are logged; 2,400 are accepted recoveries, of which 2,320 are used for post-training. Evaluation restarts every method from the fixed midpoints of 384 held-out failure intervals. Under matched actor-update counts, we compare behavior cloning of recoveries, value-based offline learning on recoveries and failed rollouts, and continued training on existing demonstrations. Within 1,200 steps on the 240 L1-L3 held-out failures, cloning improves recovery by 29.4 percentage points (pp) over the demonstration-only control; the value-based learner does not establish a further gain (1.5 pp). In exploratory evaluation from L1-L5 nominal starts at the same horizon, cloning loses 30.0 pp of success relative to the base policy; mixing in demonstrations reduces the loss to 16.5 pp, a reduction that shrinks under a stricter, pre-specified horizon. Restorable failure states and a shared evaluator let all methods be compared from identical starts.

==> figures/figure_value_guard.tex <==
\makeatletter
\newcommand\fpx@guard[3]{%
  \edef\fpx@guard@actual{\detokenize\expandafter\expandafter\expandafter{\csname #2\endcsname}}%
  \edef\fpx@guard@expected{\detokenize{#3}}%
  \ifx\fpx@guard@actual\fpx@guard@expected\else
  \expandafter\gdef\csname fpx@stale@#1\endcsname{#2}\fi}
\newcommand\fpxFigureGuard[1]{\@ifundefined{fpx@stale@#1}{}{\todohl{[Fig.~#1 shows hard-coded values that no
  longer match the result macros; update its TikZ source and re-run scripts/make\_figure\_guard.py.]}}}
\fpx@guard{1}{nFailReleased}{629\xspace}
\fpx@guard{1}{nAttemptsAll}{2,823\xspace}
\fpx@guard{1}{nAccepted}{2,400\xspace}
\fpx@guard{1}{nFailTest}{384\xspace}
\fpx@guard{1}{nFamilies}{10\xspace}
\fpx@guard{1}{framesPerFailure}{10\xspace}
\fpx@guard{1}{horizonMain}{1,200\xspace}
\fpx@guard{2}{nRolloutsGen}{11{,}190\xspace}
\fpx@guard{2}{nCandidates}{1{,}805\xspace}
\fpx@guard{2}{nShipped}{1,287\xspace}
\fpx@guard{2}{nFailReleased}{629\xspace}
\fpx@guard{2}{nFailTrain}{245\xspace}
\fpx@guard{2}{nAttemptsAll}{2,823\xspace}
\fpx@guard{2}{nAccepted}{2,400\xspace}
\fpx@guard{2}{nTrainAccPost}{2,320\xspace}
\fpx@guard{2}{nFailTest}{384\xspace}
\fpx@guard{2}{nTestConfirm}{240\xspace}
\fpx@guard{2}{nTestDiag}{144\xspace}
\fpx@guard{2}{nNominal}{500\xspace}
\fpx@guard{2}{nNormValid}{437\xspace}
\fpx@guard{2}{framesPerFailure}{10\xspace}
\fpx@guard{2}{horizonMain}{1,200\xspace}
\makeatother

